LabApprentice: Towards Harness-Level Recursive Self-Improvement for Wetlab Robotics

Wetlab robotics is a demanding setting for self-improving agents. Physical experiments take time and consume materials, leaving limited opportunities for trial and error. A wetlab measurement can tell the agent whether a procedure met its target, but not necessarily where it went wrong. We introduce LabApprentice, a wetlab robotics harness in which a coding agent recursively improves at the harness level. Without robot demonstrations, and without changing the model weights, the agent accumulates executable tools, written skills and bench measurements in a skill store that each run extends for the next. Our key insight is to use the laboratory's own instruments, unmodified, as step-level verifiers that confirm or refute a claim the agent records after each experimental step. On a Kinova Gen3 arm, we evaluate five tasks spanning common laboratory operations, including liquid handling, heating, vessel manipulation, and electrical measurement. We rerun each repeated task under a changed target, position or vessel orientation and compare against controls that start from an empty store. The agent measured the liquid that still arrived after a pour had stopped, stored a rule to stop that much earlier, and wrote a potentiostat program during execution. Agent-and-robot time fell by 22-59% from the first to the last run of each repeated task, and single empty-store controls of pouring and splitting took 1.6-3.5x as long as the runs they repeated. The last task, a four-hour hydrogel workflow, combined the programs developed in the earlier tasks. The two resulting gels had conductivities of 0.71 and 1.12 S/m, within the range reported for similar hydrogels, and a gel prepared by hand from the same recipe measured 0.71 S/m. These results show that programs developed through separate physical experiments can be reused and composed to execute a complete wetlab workflow.

==> preamble.tex <==
\usepackage[letterpaper,margin=1in]{geometry}
\usepackage[T1]{fontenc}
\usepackage{newtxtext,newtxmath}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{longtable}
\renewcommand{\topfraction}{0.85}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.75}
\usepackage{multirow}
\usepackage{array}
\usepackage{xcolor}
\usepackage{url}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage[hidelinks]{hyperref}

\newcommand{\tbd}[1]{\textcolor{red}{[TBD: #1]}}
\newcommand{\verify}[1]{\textcolor{orange}{[VERIFY: #1]}}
\newcommand{\dnote}[1]{\textcolor{blue}{[Note: #1]}}
\newcommand{\maybefig}[2]{\IfFileExists{#2}{\includegraphics[#1]{#2}}{%
  \fbox{\parbox{0.95\linewidth}{\centering\vspace{6mm}\textcolor{red}{Figure pending:
  \texttt{\detokenize{#2}}}\vspace{6mm}}}}}
\newcommand{\task}[1]{\textsc{#1}}

